Pre-train, Self-train, Distill: A simple recipe for Supersizing 3D Reconstruction

Our work learns a unified model for single-view 3D reconstruction of objects from hundreds of semantic categories. As a scalable alternative to direct 3D supervision, our work relies on segmented image collections for learning 3D of generic categories. Unlike prior works that use similar supervision but learn independent category-specific models from scratch, our approach of learning a unified model simplifies the training process while also allowing the model to benefit from the common structure across categories. Using image collections from standard recognition datasets, we show that our approach allows learning 3D inference for over 150 object categories. We evaluate using two datasets and qualitatively and quantitatively show that our unified reconstruction approach improves over prior category-specific reconstruction baselines. Our final 3D reconstruction model is also capable of zero-shot inference on images from unseen object categories and we empirically show that increasing the number of training categories improves the reconstruction quality.

==> intro.tex <==
\section{Introduction}
%Para 1 -- talk of 3D and diversity. That we see objects in 3D and the 10k categories exist. Gotta reconstruct them all!
We live in a rich, diverse world comprising of a variety of objects, from naturally occurring birds and bears, to ingeniously engineered cars and airplanes, or the pragmatically simple cups and vases. However, among the tens of thousands of object categories that exist around us, the state-of-the-art single-view reconstruction systems are only capable of inferring the 3D structure for a handful among these.

One reason for this poor scalability of 3D prediction methods is the difficulty of obtaining 3D supervision for images of generic objects. To enable learning despite this, a number of recent works \todo{cite} have instead investigated learning 3D inference using only image collections and 2D annotations (such as foreground masks) as supervisory signal. However, as these approaches learn category-level models from scratch, they need to leverage additional constraints or regularization to make learning tractable. Unfortunately, this either restricts their applicability to generic classes \eg commonly used linear morphable models cannot capture categories with large variation \todo{cite}, or makes the training process unstable \eg when using adversarial constraints \todo{cite}. Moreover, as the category-specific 3D reconstruction models are learned independently, they are unable to benefit from the common structure across objects \eg buses and toasters are both cuboidal. 
%However, these methods typically need to enforce additional constraints, such as limited intra-category shape variation to make learning tractable. 
%Para 2 -- scalable learning required, so people have used unsupervised. But still do things in a category-specific way and categories are treated independently. But categories do have things in common, and some 3D data exists.

In this work, we instead train a \emph{single} model to reconstruct objects across hundreds of diverse object categories. Towards this, we propose a simple and scalable  approach that allows learning such a unified model using in-the-wild image collections. First, we build on the pragmatic observation that synthetic 3D training data for \emph{some} categories does exist, and that this could help learn 3D prediction for \emph{new} categories given just image collections. In particular, instead of learning category-specific models from scratch, we adapt a base model trained on synthetic data to reconstruct novel categories from image collections, and show that this obviates the need for additional regularization such as limited intra-class variation or adversarial priors. We then distill the per-category adapted models into a unified high-capacity 3D reconstruction network which is finally able to reconstruct objects from across hundreds of object categories (see \figref{teaser}). Interestingly, not only can this unified model better reconstruct the categories seen during training, it can even be used for \emph{zero-shot} 3D prediction for objects from \emph{unseen} categories -- something that prior  per-category learning methods are fundamentally incapable of.
%Para 3 -- our contribution is to provide a simple recipe for scalable learning from image collections. Two steps: adapt to single categories, and distill. Using some 3D prior helps learning because initial solutions are not bad.

% Maybe the para below should be in conclusion?
We believe that our work is a step towards the goal of generic 3D reconstruction systems and that our results suggest the community should reexamine some common practices in unsupervised 3D learning. Instead of learning 3D from image collections from scratch while designing priors to prevent degenerate solutions, we find that the simpler solution of adapting a model with some 3D knowledge can suffice even when learning new categories. We also show that learning a unified model that reconstructs many categories in an unsupervised manner is not only feasible, but also beneficial, and hope that this prompts future methods to learn similar unified reconstruction models.
%\todo{one para on results + importance}
%Para 4 -- what this enables. Compared to prior work, many more classes and no templates etc. Also, better reconstruction, and show results on many classes.

==> intro1.tex <==
\section{Introduction}
We live in a rich, diverse world comprising of a variety of objects, from naturally occurring birds and bears, to ingeniously engineered cars and airplanes, or the pragmatically simple cups and vases. While we have made significant advances in semantic understanding of the
visual world which can recognize hundreds and thousands of these, state-of-the-art single-view reconstruction systems are only capable of inferring the 3D structure for a handful among these. Why is that? What leads to huge gap between the two areas?

One reason for this poor scalability of 3D prediction methods is the difficulty of obtaining 3D supervision for images of generic objects. To enable learning despite this, a number of recent works \todo{cite} have instead investigated learning 3D inference using only image collections and 2D annotations (such as foreground masks) as supervisory signal. However, as these approaches learn category-level models from scratch, they have no 3D priors and hence need to leverage additional constraints or regularization to make learning tractable. Unfortunately, this either restricts their applicability to generic classes \eg commonly used linear morphable models cannot capture categories with large variation \todo{cite}, or makes the training process unstable \eg when using adversarial constraints \todo{cite}. 

So why does recognition scales better than single-view reconstruction and can we borrrow some ideas to bridge the gap. First, we observe that while semantic recognition approaches train one model to detect hundreds of categories; single-view reconstruction approaches train one model for each category. This bottlenecks the sharing primitives and features across multiple categories. We argue this sharing is critical for generalization. In this work, we propose to train a \emph{single} model to reconstruct objects across hundreds of diverse object categories.  But there is a side-effect of using a single model for all categories -- when learned with weak supervision, there is a likely averaging effect which might cause loss of finer details. In order to avoid that, we use a two step process: first fit a category specific model followed by a distillation process to learn a joint model that provides better generalization. Finally, this still doesnt handle the 3D priors needed to regularize the model. We note that most semantic task models regularize via separating the pre-training and finetuning stages. Inspired by this, we make the pragmatic observation that synthetic 3D training data for \emph{some} categories does exist, and this small amount of 3D data could help us learn priors which can regularize learning 3D prediction for \emph{new} categories given just image collections. 

Our final approach is simple and scalable. We first pretrain a 3D reconstruction model using the 3D data from ShapeNet categories. This pre-training stage helps the model learn right 3D priors to learn from weak mask supervision. One we learn.a pre-trained base model, we then adapt this base model trained on synthetic data to reconstruct novel categories from image collections, and show that this obviates the need for additional regularization such as limited intra-class variation or adversarial priors. In the final step, we then distill the per-category adapted models into a unified high-capacity 3D reconstruction network which is finally able to reconstruct objects from across hundreds of object categories (see \figref{teaser}). Interestingly, not only can this unified model better reconstruct the categories seen during training, it can even be used for \emph{zero-shot} 3D prediction for objects from \emph{unseen} categories -- something that prior  per-category learning methods are fundamentally incapable of.





% Maybe the para below should be in conclusion?
We believe that our work is a step towards the goal of generic 3D reconstruction systems and that our results suggest the community should reexamine some common practices in unsupervised 3D learning. Instead of learning 3D from image collections from scratch while designing priors to prevent degenerate solutions, we find that the simpler solution of adapting a model with some 3D knowledge can suffice even when learning new categories. We also show that learning a unified model that reconstructs many categories in an unsupervised manner is not only feasible, but also beneficial, and hope that this prompts future methods to learn similar unified reconstruction models.
%\todo{one para on results + importance}
%Para 4 -- what this enables. Compared to prior work, many more classes and no templates etc. Also, better reconstruction, and show results on many classes.
